Stochastic Frank-Wolfe for Constrained Finite-Sum Minimization

We propose a novel Stochastic Frank-Wolfe (a.k.a. conditional gradient) algorithm for constrained smooth finite-sum minimization with a generalized linear prediction/structure. This class of problems includes empirical risk minimization with sparse, low-rank, or other structured constraints. The proposed method is simple to implement, does not require step-size tuning, and has a constant per-iteration cost that is independent of the dataset size. Furthermore, as a byproduct of the method we obtain a stochastic estimator of the Frank-Wolfe gap that can be used as a stopping criterion. Depending on the setting, the proposed method matches or improves on the best computational guarantees for Stochastic Frank-Wolfe algorithms. Benchmarks on several datasets highlight different regimes in which the proposed method exhibits a faster empirical convergence than related methods. Finally, we provide an implementation of all considered methods in an open-source package.

==> lemma_3_submitted.tex <==
\begin{lemma}\label{lemma:ht_asymptotics}
Let $\gamma_t = \frac{2}{t+2}$. We have the following bound on the expected error $\EE H_t$, for $t\geq 6$: 

\begin{align}
\bsp
    \EE H_t \leq& 2{LD_1}\left(1-\frac{1}{n}\right)^{t/2}\left(\log t + \frac{2n^2}{n-1}~\frac{1}{t+2}\right)\\
    &+ \left(1-\frac{1}{n}\right)^t H_0.
\esp
\end{align}

\end{lemma}

\begin{remark}
Our gradient estimator's error in $\ell_1$ norm vanishes faster than any polynomial. This rate depends on the assumption of the separability of $f$ into a finite sum of $L$-smooth $f_i$'s. In particular, it does not require that each $f_i$ be convex.
\end{remark}

\begin{proof}
Consider a general sequence of positive numbers, $u_1,u_2,\ldots,u_t\in\RR_+$ where for all $t$, the following recurrence holds:

\begin{align}
    u_t \leq \rho\left(u_{t-1} + \frac{K}{t+1}\right)
\end{align}
where $0<\rho<1$ and $K>0$ are scalars.

First note that all the iterates are positive. Suppose $t\geq 6$,

\begin{align*}
    u_t &\leq \rho^t u_0 + K\sum_{k=1}^t \rho^{t-k}\frac{1}{u+1} \\
    &\leq \rho^t u_0 + K \left(\sum_{k=1}^{\floor{t/2}}\rho^{t-k}\frac{1}{k+1} + \sum_{k=\floor{t/2}+1}^t\rho^{t-k}\frac{1}{k+1}\right) \\
    &\leq \rho^t u_0 + K \left(\rho^{t/2} \sum_{k=1}^{\floor{t/2}} \frac{1}{k+1} + \frac{2}{t+2} \sum_{k=\floor{t/2}+1 }^t \rho^{t-k}\right).
\end{align*}

To go from the second line to the third line, we observe that for ``old" terms with large steps sizes, we are saved by the higher power in the geometric term.
For the more recent terms, the step-size is small enough to ensure convergence. More formally, in the early terms ($1\leq k\leq \floor{t/2}$), we upper bound $\rho^{t-k}$ by $\rho^{t/2}$. In the later terms ($\floor{t/2}+1\leq k\leq t$), we upper bound $\frac{1}{k+1}$ by $\frac{2}{t + 2}$.

To obtain the full rate, we now study both parts separately. For the first part, we use knowledge of the harmonic series:

\begin{align}
    \rho^{t/2} \sum_{k=1}^{\floor{t/2}} \frac{1}{k+2} \leq \rho^{t/2}\log\left(\frac{t}{2}+3\right)
\end{align}
for $t\geq 6$, we can upper bound $\log\left(\frac{t}{2}+3\right)$ by $\log t$.

For the second part, we use knowledge of the geometric series:

\begin{align}
    \sum_{k=\floor{t/2}}^t \rho^{t-k} &\leq \frac{\rho^{(t-2)/2}}{1-\rho}
\end{align}

since $0\leq \rho^t$ and $(t-2)/2 \leq \floor{t/2}$

Finally,  for $t\geq 6$
\begin{align}
    0\leq u_t \leq K\rho^{t/2}\left(\log t + \frac{2}{\rho(1-\rho)}~\frac{1}{(t+2)}  \right) +  \rho^t u_0.
\end{align}

The error $H_t$ verifies our general conditions with $u_0 = H_0 = \|\balpha_0 - \nabla f(\XX\ww_{-1})\|_1$, defining $\ww_{-1} \defas \ww_0$ for the needs of the proof;  $\rho = 1 - \frac{1}{n}$ and $K=2{LD_1}$. Specifying these values gives us the claimed bound.
\end{proof}

==> scratch.tex <==

\section*{Scratch}

Let
\begin{equation}
    \tau_t \defas a_t \Lambda_t + c_t H_t
\end{equation}
Then we have
\begin{align}
    \EE_t \tau_t - \tau_{t-1}
\end{align}

\begin{align}
\bsp
    a_t \Lambda_t + c_t H_t \leq~&  a_t (1-\gamma_t)\Lambda_{t-1} + a_t\gamma_t^2\frac{LR_2^2}{2}  + a_t\gamma_t R_\infty \EE_t \| \nabla f(\XX\ww_{t-1}) - \balpha\|_1. + c_t \EE H_t\\
    &\leq  a_t (1-\gamma_t)\Lambda_{t-1} + a_t \gamma_t^2\frac{LR_2^2}{2}  + a_t \gamma_t R_\infty \left(1 - \frac{1}{n} \right)\left(H_{t-1} + \gamma_{t-1} L R \right) + {\blue XXXX}\\
    &\leq a_t (1-\gamma_t)\Lambda_{t-1} + a_t \gamma_t \left(1 - \frac{1}{n} \right) R_\infty  H_{t-1}  + \gamma_t^2\frac{LR_2^2}{2} + \gamma_t \gamma_{t-1} L R R_\infty
\esp
\end{align}


\begin{align}
    f(\XX \ww_t)    \leq& f(\XX\ww_{t-1})  + \gamma_t \langle \nabla f(\XX\ww_{t-1}), \XX(\sss_t - \ww_{t-1})\rangle + \gamma_t   D_2\|\nabla f(\XX\ww_{t-1}) - \balpha_t\| + \gamma_t^2\frac{LD^2_2}{2}
\end{align}

Idea: we could split the first product into two terms: one will become the contraction, and the otherone can give us terms in $ - \gamma_t \|\nabla f(\XX \ww_{t-1}) - \nabla f(\XX \zz)\|{\blue ^2}$ for some $\zz$ of our choice plus some terms in $f(\XX \ww) - f(\XX \zz)$.

==> thanks.tex <==
Comments on the draft:

- Yi Sun
- Sara Fridovich Keil
- Nicolas Le Roux

Comments on abstract:

- Yana Hasson
- Nilesh Tripuraneni
- Dhruv Sharma

Don Goldfarb for encouragement? @Fabian (sure, better be inclusive, specially in ack!)
